ASYNC: A Cloud Engine with Asynchrony and History for Distributed Machine Learning

ASYNC is a framework that supports the implementation of asynchrony and history for optimization methods on distributed computing platforms. The popularity of asynchronous optimization methods has increased in distributed machine learning. However, their applicability and practical experimentation on distributed systems are limited because current bulk-processing cloud engines do not provide a robust support for asynchrony and history. With introducing three main modules and bookkeeping system-specific and application parameters, ASYNC provides practitioners with a framework to implement asynchronous machine learning methods. To demonstrate ease-of-implementation in ASYNC, the synchronous and asynchronous variants of two well-known optimization methods, stochastic gradient descent and SAGA, are demonstrated in ASYNC.

==> Algorithms.tex <==
\subsection{SGD}







==> Draftv2.tex <==


%how we want to sell the framework
%how other papers motivate their frameworks




%  \section{Introduction}
 




 







%These problems can be solved via highly concurrent update mechanisms that expose, in effect, read-write race conditions [\citationneeded]. Empirically, on single-node systems,these asynchronous algorithms have yielded order-of-magnitude improvements in performance and are the subject of active research. Consequently, evaluation of these new asynchronous algorithms have been largely confined to single-node, multi-processor context [\citationneeded,cop].





%our processing pipeline uses Spark as a compute engine  data access. Spark is an in-memory MapReduce framework which minimizes I/O accesses .Moreover, Spark is efficient at iterative computations and is thus well-suited for the development of large-scale machine learning applications. unlike works such as ** Hadoop and Spark (which are systems that support MapReduce) provide strong operational correctness guarantees via robust fault-tolerant systems.



 %Consider  ASGD algorithm  for optimizing a least squareCurrent frameworks such as ** and ** can not be used for implementing this method because **. Also, frameworks such as ** are incapable due to **. However, we propose useful information alongside the gradient computation that supports implementing the current asynchronous optimization methods. We provide * and ***. 
 


% what are they and how?>> needs to be cleaned. explained :

% 1) Instead of forcing the user to adopt one particular dependency that may be illsuited to the problem, the \framework gives the algorithm designer flexibility in defining consistency models using \subsettaskscheduling instead of specifying dependencies using dependency graphs among individual tasks \citationneeded. This is a substantial difference to other machine learning systems.



 



% \section{framework}
%  \subsection{\subsettaskscheduling}
%  the server sends jobs to workers when at least a percentage of the workers have finished their jobs.
 
%  \subsection{consistency model}
%  We propose an upper bound for staleness in asynchronous optimization methods based on the subset task scheduling parameter.
 
%  \subsection{workers state}
%  we pass some useful information along with gradient vectors, such as historical gradients and a metadata containing info about the worker like its index and time step. 
 
%  \subsection{adaptive hyperparameter selection}
 
 





 







==> Extra.tex <==

%building blocks of \framework{} are three components  these applications while retaining the scalability and fault tolerance of
%MapReduce is a framework that enables the implementation of asynchronous optimization methods. %By offering the greatest
%degree of flexibility in designing barrier controls, selecting hyperparameters and necessary tools for implementing asynchronous methods, \framework facilitates the implementation of building blocks of asynchronous optimization methods.
%\framework{} consists of three main components that facilitate the implementation of asynchronous optimization methods. It enables the implementation of a variety of \textit{barrier control policies} to balance algorithmic convergence and system efficiency. Also, \framework implements communication efficient broadcasting strategies that facilitate the computation of \textit{historical gradients}, commonly used in a class of asynchronous optimization methods such as variance-reduced ***. Finally, workers in \framework communite their internal attributes such as staleness during the runtime to the master which will enable \textit{adaptive hyperparameter selection} used in *** optimization methods such as *** for staleness-aware a.k.a delay-tolerant asynchronous methods. First, we discuss three key features of asynchronous methods that are not supported in current frameworks. Then we present the key components of \framework that enable implementing these feature in the cloud environment.

% \textbf{Enabling dynamic hyperparameter selection:}Communication channel expose the task results and its corresponding metadata to enable users to design their dynamic hyperparameters. For example, a staleness-aware method discussed in [\citationneeded] can be implemented by using the metadata and scaling the learning rate according to the gradient staleness.

%   In distributed learning, the networked nodes have to work collaboratively to update the model parameters, and the way how they proceed is referred to as barrier control which its design has direct impact on the performance and accuracy of the system. [add delay/staleness]. Meanwhile, recent improvements on asynchronous SGD methods share two common features that makes their implementations in current frameworks inefficient if not impossible. First, variance reduced SGD algorithms such as ASAGA \cite{defazio2014saga} overcome the slow convergence of ASGD  and achieve linear convergence rate  by memorizing the gradients computed in previous iterations. However, the table containing historical gradeints can grow in size and get as big as input data which can become a substantial bottleneck \citationneeded. Second, asynchronous optimization methods such as AdaDelay \cite{sra2015adadelay} and \cite{zhang2015staleness, mcmahan2014delay} propose a gradient method where learning rates are chosen to be sensitive to the actual delay of the incoming gradients. These methods, dynamically select their hyperparamters such as learning rate based on each worker's staleness. which currently is not supported in state-of-the-art frameworks. 


% framework overview: here is an overview.we've added these components that work together to allow this to happens. These components ar e 1 2 3 which interact with each other and what they do. This how the algorithmic feature are implemented. three subsection> 


in distributed learning, the networked nodes have to work collaboratively to update the model parameters, and the way how they proceed is referred to as barrier control. Synchronous parallel protocol is practically the building block of all distributed learning frameworks, and its design has direct impact on the performance and convergence. Due to limitation of current frameworks, users have to stick to a set of pre-defined barrier controls that might be incompatible with the optimization problem.
    
    
    Stale Synchronous Parallel (SSP) [4] and Asynchronous Parallel (ASP) [2]. 
    \color{blue}
    
    
    SSP:where workers synchronize at the end of each iteration and will not proceed until the model parameters have been fully updated by all workers.
    
    ASP:where workers immediately start
    the next iteration before receiving the latest parameters.
    
    SSP:In the SSP model,
workers synchronize only when the staleness of parameters
(measured by the number of missing updates from stragglers)
exceeds a certain threshold.
    
    Therefore, increasing asynchrony is
known to increase the staleness, bringing additional deviation during training and leading
to a poorer convergence. Another way to look at the pros and cons of asynchrony is that
increasing asynchrony improves hardware efficiency as it takes a shorter time for each
system to perform each iteration, and worsens statistical efficiency as it requires more
    
     These are algorithms whose purpose is to determine if a worker should proceed to the next iteration of a computation or
if it should wait. The most dominant schemes are Bulk Synchronous Parallel (BSP) [11],
Stale Synchronous Parallel (SSP) [4] and Asynchronous Parallel (ASP) [2].

    Probabilistic Synchronous Parallel (PSP)  introduces a random sampling  .when making barrier control decisions, PSP makes decisions based on sampled
states. Through sampling, PSP is more resistant to stragglers as compared to the other
barrier controls, improving robustness. Furthermore, PSP improves scalability as it does
not require a view of the global state and it strikes a balance between efficiency and
accuracy.

PSP is able to improve convergence speed and iteration
throughput of traditional barrier control methods.



These methods reduce the variance of the noise caused by the sampling from training data Historical gradeints are also used to reduce the  However, the table containing historical gradients can grow in size and get as big as input data which can become a substantial bottleneck.

In this paper, we propose a general remedy to the “noisy gradient” problem ubiquitous to all stochastic
gradient optimization algorithms for different models. Our approach builds on a variance reduction
technique, which makes use of control variates [3] to augment the noisy gradient and thereby reduce
its variance.it uses the noisy gradient
computed from the random data samples instead of the true gradient computed
from the entire datase
    
    
    





% In order to faciltate the implementation of the barrier control, scheduler takes a user-defined function that 

% In general, there are three major barrier controls: Bulk synchronous parallel (BSP), Stale synchronous parallel (SSP), and Asynchronous parallel (ASP). These three barrier control are currently implemented in the \framework{}. However, recent barrier policies for large scale machine learning problems could be added to \framework{}, as long as the required algorithm-specific scheduler can be described in this manner as well.

% the task scheduling through user-defined function.  \framework{} allows the server node to keep track of the workers activity through the communication channel. An asynchronous method can decide how inactive (or active) workers can proceed which directly affects its convergence and system efficiency.


 
 
 
 
 
 
 
 
 
 
 
 

 
 






\textbf{Implementing barrier control}
\textbf{Implementing historical gradients}
\textbf{Implementing dynamic hyperparameters}



% \subsection{Communication channel/context}
% The communication channel is the main building block of \framework{} that provides the necessary tools and information regarding workers tasks and internal attributes of each worker.

 


% Since each worker's task result that arrives at the master node corresponds to previous iterations, it can not reflect current worker's status such as most recent staleness or it's status of being \textit{active}, currently processing a task, or \textit{inactive}. Therefore, task results and workers' status represent different information, the former one created and submitted by workers and used to update the model parameter, while the latter one is handled by the master node and used to define barrier controls. Communication channel decouples these information and updates them separately in order to facilitate developing the key features of asynchronous methods. 

% Communication channel facilitates developing asynchronous methods through i) workers activity[looking for name] status : each worker is associated with a set of attributes such as its current staleness that can be used through out developing asynchronous optimization methods. ii) ResultHolder [looking for name] containing the gradient vectors as they arrive and tags them with the gradient staleness and the worker index. 



% we broadcast the iteration 
%  \framework{} propose a dynamic broadcasting that enables historical gradeint computations. At the beginning og each iteration, the model parameter is broadcasted to all or part of the available workers. In order to be able to implement historical gradients, workers need to use model parameter

% Different asynchronous methods can make use of historical gradients to improve their convergence rate at the cost of additional storage by memorizing a table of historical gradients on the master node. We follow a similar  idea for recomputing historical gradients in  \cite{defazio2014saga} and generalize it to stochastic gradient based optimization algorithms.

% \framework{}  proposes a dynamic broadcast variable that gives workers access to the model parameter at any previous iteration. Each worker can independently request a previous model parameter from the master node to get a read-only variable cached on its machine. If the variable already exists on the worker node, it is used to recompute the gradient without any further network communication. Otherwise the master node sends the model parameter at the specified iteration to the worker node. 

% [Where to put this?> On of the drawbacks of cloud platforms is the possible failure of the nodes which makes it challenging to recover from faults. However, Spark optimizes its computation with the assumption that these faults are unlikely to happen and uses in-memory computation to increase its performance. Therefore, a possible ASAGA implementation on Spark  that needs historical gradient computations can either store these vectors while suffering from a substantial storage cost or recompute them at the cost of extra computation overhead. On the other hand, recomputing previous gradients needs access to previous shared variables which currently requires storing previous model parameters and sending them to workers at each iteration which can become a substantial bottleneck.]








% \subsection{Dynamic Broadcasting or storage efficient broadcasting/ dynamic shared variable}Different asynchronous methods can make use of historical gradients to improve their convergence rate at the cost of additional storage by memorizing a table of historical gradients on the master node. We follow a similar  idea for recomputing historical gradients in  \cite{defazio2014saga} and generalize it to stochastic gradient based optimization algorithms.

% \framework{}  proposes a dynamic broadcast variable that gives workers access to the model parameter at any previous iteration. Each worker can independently request a previous model parameter from the master node to get a read-only variable cached on its machine. If the variable already exists on the worker node, it is used to recompute the gradient without any further network communication. Otherwise the master node sends the model parameter at the specified iteration to the worker node. 




As the magnitude of the delays gets larger and larger in the order of growth, one needs to use a more conservative step-size sequence in order to mitigate the damage done by the stale gradient information.
The class of gradient staleness-dependent method where learning rates are dynamically changed are not supported by current frameworks.
     
     \color{blue}
      \cite{zhang2015staleness} introduce a variant
of the ASGD algorithm in which they keep track of the staleness associated with each gradient computation and adjust
the learning rate on a per-gradient basis by simply dividing
the learning rate by the staleness value.

The staleness of the gradient is random, and can vary across iterations. Intuitively, if the gradient
is less stale, we want to weigh it more while updating the parameter w, and if it is more stale we
want to scale down its contribution to the update. With this motivation, \cite{dutta2018slow} proposes a new adaptive learning rate to compensate for staleness.
     \color{black}
     
     
     
     \section{Related work}

Asynchronous parallel optimization has recently become a popular way to speedup machine learning algorithms using shared memory and distributed systems. The most widely used asynchronous optimization algorithms are stochastic gradient methods \cite{dean2012large,duchi2015asynchronous,recht2011hogwild}  and coordinate descent \cite{avron2015revisiting,hsieh2015passcode,lian2015asynchronous}. An asynchronous variant of SGD with constant step size called Hogwild! was presented in \cite{recht2011hogwild} which can achieve a sub-linear convergence rate and only converges to a neighborhood of the optimal solution compard to DownpourSGD \cite{dean2012large} and PetuumSGD\cite{xing2015petuum} that guarantee the convergence to optimal solution at the expense of slower convergence rate. The asycnhronousy of these methods due to their execution model, inevitably adds staleness to the systems which leads to a poor convergence. 
Recent works mitigate the effect of stale gradeints by either changing the execution model and bounding the staleness \cite{xing2015petuum,ming2018distributed,ho2013more,agarwal2011distributed, zinkevich2009slow,cipar2013solving}  or theortitically adapting the method to the stale gradients \cite{zhang2015staleness,mcmahan2014delay}. However, recent works \cite{zhang2018adaptive,wang2017probabilistic} show that current execution models also known as barrier controls  can be improved by dynamically adjusting the communication mechanism between computational nodes and the server according to the performance of each computational node. Meanwhile, works such as \cite{zhang2015staleness,mcmahan2014delay} aim to compensae for the staleness by using a staleness-dependent learning strategy to scale the algorithm hyperparameters. Recently, many works aim at improving the convergence of SGD methods by reducing the variance of the noise introduced by randomization. works such as \cite{mania2017perturbed,ming2018distributed,reddi2015variance} periodically sycnhronize their models  in order to achieve a linear convergencce rate.  works such as ASAGA\cite{leblond2016asaga,pedregosa2017breaking} remove this extra synchronoization cost  by storing a table of historical gradient  eventhough its storage overhead can become a significant bottleneck for large scale optimization problems. A different approach for distributed and parallel optimization is based on the alternating direction method of multipliers (ADMM)\cite{boyd2011distributed} where  has been extended to the asynchronous setting for convex\cite{zhang2014asynchronous} and non-convex \cite{hong2018distributed,chang2016asynchronous} problems. Our framework provides necessary tools to support a variety of these asynchronous algorithms and allows users to develop different barrier controls, uses historical gradients to improve convergence and dynamically adapt their parameters to mitigate the staleness problem.




% Asynchronous parallel optimization has recently become a popular way to speedup machine learning algorithms using shared memory and distributed systems. The most widely used asynchronous optimization algorithms are stochastic gradient methods \cite{dean2012large,duchi2015asynchronous,recht2011hogwild}  and coordinate descent \cite{avron2015revisiting,hsieh2015passcode,lian2015asynchronous}. An asynchronous variant of SGD with constant step size called Hogwild! was presented in \cite{recht2011hogwild} which can achieve a sub-linear convergence rate and only converges to a neighborhood of the optimal solution. Methods such as DownpourSGD \cite{dean2012large} and PetuumSGD\cite{xing2015petuum} propose another variants of asynchronous SGD that to guarantee the convergence to optimal solution at the expense of slower convergence rate. Even though, the asynchronous variants of the SGD can be significantly more efficient due to their execution model, this asycnhronousy inevitably adds staleness to the systems which can lead to a poor convergence. Recent works aim to mitigate the effect of stale gradeints by either changing the execution model \cite{xing2015petuum,ming2018distributed,ho2013more,agarwal2011distributed, zinkevich2009slow,cipar2013solving}  or theortitically adapting to the stalenss \cite{zhang2015staleness,mcmahan2014delay}. Works such as \cite{xing2015petuum,cipar2013solving}  introduce stale-synchronous parallel(SSP) execution model which bounds the staleness to balance the algorithmic convegence and performance. However, recent works \cite{zhang2018adaptive,wang2017probabilistic} show that current execution models such also known as barrier controls, show poor performance  when the compuatational nodes performance can change in time. Therefore, they propose an adaptive sycnhronou  parallel method that  dynamically adjusts the communication mechanism between computational nodes and the server according to the performance of each computational node. Similarly \cite{wang2017probabilistic} propose a  probabilistic sycnhronous parallel model to increase the convergence speed and the scalability by introducing a sampling primitive into the system. Meanwhile, works such as \cite{zhang2015staleness,mcmahan2014delay} aim to compensae for the staleness by adaptively changing the parameters of the algorithms. Works such as \cite{zhang2015staleness} uses a staleness-dependent learning strategy to scale the algorithms hyperparameters according to the staleness and hence improving the convergence.  Recently, many works aim at improving the convergence of SGD methods by reducing the variance of the noise introduced by randomization. works such as \cite{mania2017perturbed,ming2018distributed,reddi2015variance} periodically sycnhronize their models  in order to achieve a linear convergencce rate.  works such as ASAGA\cite{leblond2016asaga,pedregosa2017breaking} remove this extra synchronoization cost  by storing a table of historical gradient  to reduce the variance. eventhough its storage overhead can become a significant bottleneck for large scale optimization problems. A different approach for distributed and parallel optimization is based on the alternating direction method of multipliers (ADMM)\cite{boyd2011distributed} where  has been extended to the asynchronous setting for convex\cite{zhang2014asynchronous} and non-convex \cite{hong2018distributed,chang2016asynchronous} problems. Our framework provides necessary tools to support a variety of these asynchronous algorithms and allows users to develop different barrier controls, uses historical gradients to improve convergence and dynamically adapt their parameters to mitigate the staleness problem.




% Asynchronous parallel optimization has recently become a popular way to speedup machine learning algorithms using shared memory and distributed systems. The most widely used asynchronous optimization algorithms are stochastic gradient methods\cite{dean2012large,duchi2015asynchronous,recht2011hogwild}  and coordinate descent \cite{avron2015revisiting,hsieh2015passcode,lian2015asynchronous}.  An asynchronous variant of Sgd with constant step size called Hogwild! was presented in \cite{recht2011hogwild} which can only achieve a sub-linear convergence rate. DownpourSGD \cite{dean2012large} propose a variant of asynchronous stochastic gradient descent that uses multiple replicas of a single model which periodically synchronize their results.  Similar to Downpour SGD, the PetuumSGD\cite{xing2015petuum} uses a decaying learning rate to guarantee the convergence at the expense of slower convergence to the optimal solution. Even though, the asynchronous variants of the SGD can be significantly more efficient due to their execution model, this asycnhronousy inevitably adds staleness to the systems which can lead to a poor convergence. Recent works aim to mitigate the effect of stale gradeints by either changing the execution model of the asynchronous algorithm \cite{xing2015petuum,ming2018distributed,ho2013more,agarwal2011distributed, zinkevich2009slow,cipar2013solving}  or theortitically adapting to the stalenss \cite{zhang2015staleness,mcmahan2014delay}. Works such as \cite{xing2015petuum,cipar2013solving}  introduce stale-synchronous parallel(SSP) execution model which bounds the staleness to balance the algorithmic convegence and performance. However, recent works \cite{zhang2018adaptive,wang2017probabilistic} show that current execution models such as SSP also known as barrier control policies, show poor performance in *** .Therefore \cite{wang2017probabilistic} propose a  probabilistic sycnhronous parallel model to increase the convergence speed and the scalability by introducing a sampling primitive into the system . \cite{zhang2018adaptive} claims that that SSP shows poor convergence  when the compuatational nodes performance can change in time. Therefore, they propose an adaptive sycnhronou  parallel method that  dynamically adjusts the communication mechanism between computational nodes and the server according to the performance of each computational node.  Meanwhile, works such as \cite{zhang2015staleness,mcmahan2014delay} aim to compensae for the staleness by adaptively changing the parameters of the algorithms. Works such as \cite{zhang2015staleness} uses a staleness-dependent learning strategy to scale the algorithms hyperparameters according to the staleness and hence improving the convergence. Recently, many works aim at improving the convergence of SGD methods by reducing the variance of the noise introduced by randomization. works such as \cite{mania2017perturbed, leblond2016asaga,reddi2015variance,pedregosa2017breaking,ming2018distributed} achive a linear convergence rate at the expense of computational and/or storage overhead. Methods such as \cite{mania2017perturbed,ming2018distributed,reddi2015variance} are epoc based where they have to periodically sycnhronize in order to achieve a linear convergencce rate. Therefore, they are not fully asynchronous. However, works such as ASAGA\cite{leblond2016asaga,pedregosa2017breaking} has been shown effective to reduce the variance of SGD running on a single node. However ASAGA reduces the variance by storing a table of historical gradient which can become a significant bottleneck for large scale optimization problems. A different approach for distributed and parallel optimization is based on the alternating direction method of multipliers (ADMM). Recently, the synchronous distributed ADMM \cite{boyd2011distributed},  has been extended to the asynchronous setting for convex\cite{zhang2014asynchronous} and non-convex \cite{hong2018distributed,chang2016asynchronous} problems. Our framework provides necessary tools to support a variety of these asynchronous algorithms and allows users to develop different barrier controls, uses historical gradients to improve convergence and dynamically adapt their parameters to mitigate the staleness problem.


\textbf{shared memory:
}Current  implementation of many asycnrhnous optimization methods rely on shared memory for local communication and message passing. Recent works in first order asynchrnous optimization and beyond \cite{recht2011hogwild,mania2017perturbed,de2017understanding,qin2017dot} , extending to parallel iterative linear solvers \cite{liu2014asynchronous,avron2015revisiting}, has further demonstrated that linear speedups are generically possible in the asynchronous shared-memory setting even when applied to non-convex problems \cite{dean2012large,chilimbi2014project}. Some general framework such as \cite{pan2016cyclades,nawab2017cop} propose lock-free parallelization of stochastic optimization algorithms, while maintaining serial equivalence by partitioning updates among cores, in a way that ensures that there are no conflicts across partitions. 
However, with the increase of data scale, shared-memory implementation are not efficient enough to handle large-scale datasets[]. Furthermore, in this big data era, many large-scale datasets are distributively stored on a cluster of multiple machines. Therefore,  the shared-memory implementations cannot be directly used for these kinds of distributed applications.

\textbf{distirbuted:}

The demand for large-scale computational and storage resources, has driven many to develop new parallel and distributed ML frameworks, including

\textbf{1)dataflow systems :
}Architecturally, commodity distributed dataflow systems such as Hadoop[] and Spark[] are optimized for coarse-grained (often bulk synchronous
parallel data transformations and are not designed to natively provide the fine-grained communication required for efficient asynchronous analytics tasks[hadoop,Spark,Mahout,iihadoop,i2mapreduce]. Consequesntly, machine learning libraries on these data flow systems such as MLlib iare also limited to sycnhronous algorithms[MLlib].

Recent works have tried exploiting such systems to  support asynchronou  algorithms while benefitng from theri programming models .[II hadoop] propose an extension to Hadoop[] and  performs iterative or incremental computations when data is changing over time. It accelerates program execution by performing the incremental computations on the small fraction of data that is afected by changes rather than the whole data. iiHadoop runs tasks asunchronously if the output of one task is not needed as an input to another task. However, in asycnhronous optimization methods, the tasks use the shared model as input and contribute their updates to the same shared model again. Some works such as ASIP[]  add a communication layer to Spark to enable fine-grained asynchronous communication among machines. ASIP is restricted to fully asycnhonous algorithms and can not be used to implement adpative asychnornous optimization methods such as [] and []  where workers specific data is needed. 

The closest work to us is Glint[] which provides a parameter server implementation that integrates with Spark and allows the workers to update a shared model stored on Glint parameter servers. Glint provides a communication  method that allows worker to push their updates to the shared model. However, workers are not allows to locally reduce their updates first and submit the aggregated update. Therefore, Glint does not supprt mini-batch asycnhronous optimization methods where the gradeints are reduce locally per worker. In addition, Glint only support fully asycnhronous execution model.
  



\textbf{2)parameter servers 
:}Parameter server architectures such as [**]  are widely used in distributed ML due to the fact that they adopt asynchronous or bounded asynchronous parallelism that improves efficiencyand they have wide applicability to nearly all ML models.  
 

Some Application specific works such as DistBelief [15], Project Adam [12],  were used to train deep neural networks. More general frameworks such as  Petuum[] improve[YahooLDA] with a bounded delay model while placing further constraints on the worker threading model and restricting the implementing any exectution model except stale sycnrhnous parallel. Eventhough [parameter server] was proposed to improve some of these constraints, it neither supports asycnrhnous optimization methods that rely on the worker specific attributes  such as stalenes, nor provides the flexibility of definig new barrier controls. Furthermore, [parameter server] does not provide a solution for historical gradeint computations as it requires tracking the shared model over iterations which currently is not supported.

[MLNET] designed  a communication layer that uses tree-based overlays to implement distributed aggregation and multicast and reduces network traffic. However, the server only has access to aggregated results while many asycnhronous methods[**] rely on individual task results to update the model parameter. Furthermore, MLNET require knowledge of worker and parameter server locations and, hence, it might is not suitable for public cloud deployments.

Litz  is an elastic ML framework that exposes an event-driven programming model which focuses on elasticity and resource adaptability for ML applications  which relies on coarsegrained snapshots for recovery.

Works such as [KunPeng] provides a low-level interface for developing ML algorithm without providing the flexibility of developing different execution models. Furthermore, asycnhroous methods such as [**] which rely on worker side infromation such as staleness are not supported.


Meanwhile, Peer-to-peer networks such as [Orpheus,MALT,Thrill, TMSN] present aframework for implementing machine learning algorithms that require communication among workers in order to gaurantee the convergence. However, many of the recent asycnhronous sotchastic gradient methods [**] follow parameter server archoiteure when the workers oonly communicate with the server. 

We propose a machine learning framework for asycnrohnos optimization methods that **


% general optimization function,gradient w...
%


% In the machine learning community, the statistical nature of many  optimization problems has led to increasing interest in exploiting asynchrony during computation. That is, a range of recent theoretical results has demonstrated that removing synchronization within an emerging class of problems can yield surprising improvements in performance[\citationneeded, cop]. Asynchronous parallelism has been successfully applied to speedup many state-of-the-art optimization algorithms, such as SGD \cite{lian2015asynchronous}, SVRG \cite{zhang2015fast} and SAGA (\cite{leblond2016asaga}).

%  \begin{figure}
%   \includegraphics[width=\linewidth]{Figures/frameworkFigure.jpg}
%   \caption{Framewrok architecture}
%   \label{fig:framework}
% \end{figure}
%The most straightforward implementation of mini-batch stochastic gradient descent (SGD) using map-reduce is shown in Algorithm \autoref{alg:sgd} in which the master node simply splits the workload amongst the workers at every iteration. The map phase takes in a list of key-value pairs and applies the gradient function independently on workers. The reduce phase must wait for all the map tasks to complete. Afterward, the master node aggregate the task results and update the model.  In the asynchronous counterpart, different workers should be able to send their task results to the master without coordinating with other workers  inevitably adding \textit{staleness} to the system wherein some of the workers compute gradients using model parameters that may be several gradient steps behind the most updated set of model parameters. A simplified implementation of ASGD in our \framework{} is shown in Algorithm \autoref{alg:asgd}. Other variants of the ASGD algorithm require more information from workers to perform an update. For example, the staleness-aware ASGD \cite{zhang2015staleness} defines a gradient staleness-dependent learning rate dependent on each worker staleness in each iteration. 





%[to be cleaned:]
%\begin{itemize}
 %   \item Barrier control: In distributed learning, the networked nodes have to work collaboratively to update the model parameters, and the way how they proceed is referred to as  synchronous parallel design (or barrier control). Synchronous parallel protocol is practically the building block of all distributed learning frameworks, and its design has direct impact on the performance and accuracy of the system. 
  
    
  %  \item History of gradients: 
 %   Recently, variance reduced SGD algorithms such as ASAGA \cite{defazio2014saga} have gained many attentions to solve machine learning problems where they maintain variance reduction by memorizing the gradients computed in previous iterations. They have been proposed to overcome the slow convergence of SGD  and are proved to have linear convergence rate on strongly convex smooth problem. However, the table containing historical gradeints can grow in size and get as big as input data which can become a substantial bottleneck \citationneeded. 

    
    
  %  \item Dynamic hyperparameter selection: some synchronous optimization methods adaptively select their hyperparamters such as learning rate based on the \textit{staleness} of the gradients that were evaluated at an older version of the model. Works such as AdaDelay \cite{sra2015adadelay} and \cite{zhang2015staleness, mcmahan2014delay} propose a gradient staleness-dependent method where learning rates are chosen to be sensitive to the actual delay of the incoming gradients. 
    
%    examples:




 %   The learning rate can diminish according to the delay of a worker  or the mini-batch size can gradually be increased in each iteration. 
    
 %   local states: Each worker can compute partial gradients while maintaining a set of sates that are essential for deploying many state-of-the-art asynchronous optimization methods including the batch size to use for data parallelism, local time step and clock time. This data is specific to each worker and needs to be attached to each gradient update sent to the master node.
    
%\end{itemize}

%\textbf{[Related work] from before}
%current state of the art frameworks such as ... have been used to implement ** algorithms. However, they do  not support ** 

%\cite{li2014scaling} propose a parameter server framework for general machine learning problems. However, the current framework lacks the ability to implement staleness-aware asynchronous optimization methods[\cite{mcmahan2014delay},\cite{zhang2015staleness}].  As the magnitude of the delays gets larger and larger in the order of growth, one needs to use a more conservative step-size sequence in order to mitigate the damage done by the stale gradient information. Also, new asynchronous methods such as \cite{wang2017probabilistic} that uses an probabilistic approach to control the barrier in the asynchronous SGD method can not be implemented since the workers local states is not exposed to the user. 
 
 


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)
